Artificial Intelligence for Literature Reviews: Opportunities and Challenges

This manuscript presents a comprehensive review of the use of Artificial Intelligence (AI) in Systematic Literature Reviews (SLRs). A SLR is a rigorous and organised methodology that assesses and integrates previous research on a given topic. Numerous tools have been developed to assist and partially automate the SLR process. The increasing role of AI in this field shows great potential in providing more effective support for researchers, moving towards the semi-automatic creation of literature reviews. Our study focuses on how AI techniques are applied in the semi-automation of SLRs, specifically in the screening and extraction phases. We examine 21 leading SLR tools using a framework that combines 23 traditional features with 11 AI features. We also analyse 11 recent tools that leverage large language models for searching the literature and assisting academic writing. Finally, the paper discusses current trends in the field, outlines key research challenges, and suggests directions for future research.

==> tables/LiteratureReviewTools.tex <==
\begin{table}[]
\caption{Literature Review Tools based on LLMs.\label{tab:LiteratureReviewTools}}

\resizebox{\textwidth}{!}{\begin{tabular}{l|l|l|l|l|l|c}

\toprule
\textbf{ID} & \textbf{Tool}                & \textbf{Mode} & \textbf{Approach} & \textbf{Type} & \textbf{Website} & \textbf{Reference} \\

\midrule
1           & Scite                    & Web          & Proprietary           & Search Engine    & \href{https://scite.ai/}{https://scite.ai/}          & ~\cite{nicholson2021scite,Rife2021sciteTN,brody2021scite}             \\
2           & Elicit                  & Web          & Open Source           & Search Engine    & \href{https://elicit.com/}{https://elicit.com/}          &~\cite{kung2023elicit}      \\
3           & Consensus                  & Web          & Proprietary          & Search Engine    & \href{https://consensus.app/}{https://consensus.app/}          & -             \\
4           & EvidenceHunt                  & Web          & Open Source          & Search Engine    & \href{https://evidencehunt.com/}{https://evidencehunt.com/}          & -             \\
5           & MirrorThink                  & Web          & Proprietary          & Search Engine    & \href{https://mirrorthink.ai/}{https://mirrorthink.ai/}          & -             \\
6           & Perplexity                  & Web \& App          & Open Source          & Search Engine    & \href{https://mirrorthink.ai/}{https://mirrorthink.ai/}          & -             \\
7           & Scispace                  & Web           & Open Source          & Search Engine    & \href{https://typeset.io/}{https://typeset.io/}          & -             \\
8           & Jenni.ai                  & Web \& App           & Proprietary          & Writing Assistant    & \href{https://jenni.ai/}{https://jenni.ai/}          & -             \\ 
9           & ResearchBuddies                  & Web        & Open Source          & Writing Assistant    & \href{https://researchbuddy.app/}{https://researchbuddy.app/}          & -             \\ 
10         & Silatus                  & Web        & Proprietary          & Writing Assistant    & \href{https://silatus.com/}{https://silatus.com/}          & -             \\ 
11          & Textero.ai                  & Web           & Proprietary          &Both     & \href{https://textero.ai/}{https://textero.ai/}          & -             \\



\bottomrule

\end{tabular}}
\end{table} 

==> tables/Mapping_AI_vs_SLR_features.tex <==

\begin{table}%[!h]
\caption{Mapping between the AI features and their category.\label{tab:ai_features_categorised}}
\centering
\begin{tabular}{|l|l|l|}
\toprule
\textbf{Basic}      & \textbf{Technical}  & \textbf{Support} \\
\midrule
SLR Task         & Input & Pre-screening support  \\
Approach           & Output              & Post-screening support \\
Text representation   & Model execution               &                        \\
Minimum requirement   &               &                        \\
Human Interaction &                     &         \\
Research field&                     &         \\
\bottomrule
\end{tabular}
\end{table}


==> tables/NLPTasks.tex <==
%\begin{sidewaystable}[]
\begin{table}[]


\caption{NLP sub-tasks for Screening and Extraction and their Association with  the NLP Nomenclature~\cite{schopf2023exploring}.\label{tab:nlp_tasks}}


% \resizebox{\textwidth}{!}{\begin{tabular}{l|l|l|l|l}

\begin{tabular}{p{1.2cm}|p{2cm}|p{3cm}|p{3cm}|p{3cm}}
\toprule
SLR Phase                   & Schopf Task                                              & Schopf Sub-task                                   & SLR Sub-task                                                                     & Description                                                                                                                                                                                                                                                                                                                                                                                                                         \\
\midrule

Screening  & Semantic Text Processing                & Semantic Similarity              & Classification   of relevant papers given a set of seed papers                   & It   classifies papers as relevant based on a model trained on a seed of papers   made of relevant and irrelevant scholarly documents categorised by the user.   The model uses a human in the loop approach in which it is constantly being   trained based on the inclusion of relevant or irrelevant  papers until the user decides that there is   no more papers to be categorised as relevant.                                \\
                            &                                                          &                                                   & Identification of biomedical studies based on a   pre-built classification model & It   identifies studies such as RCTs, Systematic Reviews,  Economic Evaluations,  COVID-19 categories or  long COVID based on a model trained on   biomedical data.                                                                                                                                                                                                                                                                 \\
                            & Information   Extraction \& Text Mining & Text Clustering                                   & Clustering   of Abstracts                                                        & It   groups papers according to their similarity based on the most meaningful   words and  their synonyms  found within the abstracts.                                                                                                                                                                                                                                                                                              \\
                            &                                                          & Name Entity Recognition and Text   Classification & Identification   of the category attributed to the paper by the user             & It   identifies the user-assigned category (tag) of the full-text document   determined as relevant in the screening phase.                                                                                                                                                                                                                                                                                                         \\ \hline
Extraction & Information Extraction \&   Text Mining & Text Classification                               & Identification   of risk of bias                                                 & It   identifies potential sentences of a full-text document as having a low, high   or  unclear risk of bias based on the   Cochrane Risk of Bias tool.                                                                                                                                                                                                                                                                             \\
                            &                                                          & Name Entity Recognition and Text   Classification & Name Entity Recognition (NER)                                                    & It   identifies entities (e.g., population, intervention, sex ) for RCTs, animal   studies or the ones the  users wants   the model to extract.  The RCTs are   based on the 21 categories listed on the Consolidated Standards of Reporting   Trials (CONSORT). Whereas, the animal studies entities identifies animal   models (species, strain, and sex),exposures, experiments and endpoints (organ   tissues, health effects). \\
                            &                                                          & Relation Extraction                               & Entity   Linking                                                                 & It   establishes connections between animal studies entities or the ones define by   the user based on entities previously established by him. In the former, the   model  determines the   relationships of  experiments with endpoints or experiments   with animal models and exposures.                                                                                                 \\                                                                                                                                             
\bottomrule
\end{tabular}
%\end{tabular}}

%\end{sidewaystable}
\end{table}
\begin{table}[]
\begin{tabular}{ll}
SLR   Sub-task                                                                   & Description                                                                                                                                                                                                                                                                                                                                                                                                                         \\
Classification of relevant papers given a set of seed papers                     & It   classifies papers as relevant based on a model trained on a seed of papers   made of relevant and irrelevant scholarly documents categorised by the user.   The model uses a human in the loop approach in which it is constantly being   trained based on the inclusion of relevant or irrelevant  papers until the user decides that there is   no more papers to be categorised as relevant.                                \\
Identification of biomedical studies based on a pre-built   classification model & It   identifies studies such as RCTs, Systematic Reviews,  Economic Evaluations,  COVID-19 categories or  long COVID based on a model trained on   biomedical data.                                                                                                                                                                                                                                                                 \\
Clustering of Abstracts                                                          & It   groups papers according to their similarity based on the most meaningful   words and  their synonyms  found within the abstracts.                                                                                                                                                                                                                                                                                              \\
Identification of the category attributed to the paper by the   user             & It   identifies the user-assigned category (tag) of the full-text document   determined as relevant in the screening phase.                                                                                                                                                                                                                                                                                                         \\
Identification of risk of bias                                                   & It   identifies potential sentences of a full-text document as having a low, high   or  unclear risk of bias based on the   Cochrane Risk of Bias tool.                                                                                                                                                                                                                                                                             \\
Name Entity Recognition   (NER)                                                  & It   identifies entities (e.g., population, intervention, sex ) for RCTs, animal   studies or the ones the  users wants   the model to extract.  The RCTs are   based on the 21 categories listed on the Consolidated Standards of Reporting   Trials (CONSORT). Whereas, the animal studies entities identifies animal   models (species, strain, and sex),exposures, experiments and endpoints (organ   tissues, health effects). \\
Entity Linking                                                                   & It   establishes connections between animal studies entities or the ones define by   the user based on entities previously established by him. In the former, the   model  determines the   relationships of  experiments with endpoints or experiments   with animal models and exposures.                                                                                                                                        
\end{tabular}
\end{table}

==> tables/NLPTasksDescription.tex <==
%\begin{sidewaystable}[]
\begin{table}[]


\caption{Description of the SLR Tasks. \label{tab:nlp_tasks_description}}


% \resizebox{\textwidth}{!}{\begin{tabular}{l|l|l|l|l}

\begin{tabular}{p{4.5cm}|p{7cm}}
%\begin{tabular}{l|l}

\toprule
\textbf{SLR Task}                                                                   & \textbf{Description}                                                                                                                                                                                                                                                                                                                                                                                                                         \\
\midrule
Classification of relevant papers given a set of seed papers                     & It   classifies papers as relevant based on a model trained on a seed of papers   made of relevant and irrelevant scholarly documents categorised by the user.   The model uses a human in the loop approach in which it is constantly being   trained based on the inclusion of relevant or irrelevant  papers until the user decides that there is   no more papers to be categorised as relevant.                                \\
\midrule
Identification of biomedical studies based on a pre-built   classification model & It   identifies studies such as RCTs, Systematic Reviews,  Economic Evaluations,  COVID-19 categories or  long COVID based on a model trained on   biomedical data.                                                                                                                                                                                                                                                                 \\
\midrule
Clustering of Articles                                                          & It   groups papers according to their similarity based on the most meaningful   words and  their synonyms  found within the abstracts.                                                                                                                                                                                                                                                                                              \\
\midrule
Identification of the category attributed to the paper by the   user             & It   identifies the user-assigned category (tag) of the full-text document   determined as relevant in the screening phase.                                                                                                                                                                                                                                                                                                         \\
\midrule
Identification of risk of bias                                                   & It   identifies potential sentences of a full-text document as having a low, high   or  unclear risk of bias based on the   Cochrane Risk of Bias tool.                                                                                                                                                                                                                                                                             \\
\midrule
Name Entity Recognition   (NER)                                                  & It  identifies specific entities from the text that can be either predetermined (e.g., RCT entities) or defined by the users.

%for RCTs, animal   studies or the ones the  users wants   the model to extract.  The RCTs entities are   based on the 21 categories listed on the Consolidated Standards of Reporting   Trials (CONSORT)~\cite{moher2001consort}. Whereas, the animal studies\tnote{*} entities identifies animal   models (species, strain, and sex),exposures, experiments and endpoints (organ   tissues, health effects). \\
\midrule
%Entity Linking                                                                   & It   establishes connections between animal studies entities or the ones defined by   the user based on entities previously established by him. In the former, the   model  determines the   relationships of  experiments with endpoints or experiments   with animal models and exposures.                                                                             \\

\bottomrule                                                       
\end{tabular}

\smallskip\footnotesize
%\begin{tablenotes}
%    \item[*] It identifies entities such as test article, species, strain, sex, route of administration, vehicle, dose amount, dose unit, dose frequency, dose duration, time of dose, organ/tissue, effect , result, statistical test,  p-value, table number, figure number.   
%\end{tablenotes}

\end{table}



==> tables/NLPTasksMapping.tex <==

%\begin{sidewaystable}[]
\begin{table}[]

\caption{NLP sub-tasks for Screening and Extraction and their Association with  the NLP Nomenclature~\cite{schopf2023exploring}.\label{tab:nlp_tasks_mapping}}

% \resizebox{\textwidth}{!}{\begin{tabular}{l|l|l|l|l}
%\begin{tabular}{p{4.5cm}|p{7cm}}
\begin{tabular}{p{1.5cm}|p{2cm}|p{2.5cm}|p{5cm}}

\toprule



SLR Phase                   & Schopf Task                                              & Schopf Sub-task                                   & SLR Sub-task                                                                     \\

\midrule
Screening  & Semantic Text Processing                & Semantic Similarity              & Classification   of relevant papers given a set of seed papers                   \\ \cline{4-1}
                            &                                                          &                                                   & Identification of biomedical studies based on a   pre-built classification model \\\cline{4-2}
                            & Information   Extraction \& Text Mining & Text Clustering                                   & Clustering   of Abstracts                                                        \\\cline{4-3}
                            &                                                          & NER and Text   Classification & Identification   of the category attributed to the paper by the user             \\ \hline
Extraction & Information Extraction \&   Text Mining & Text Classification                               & Identification   of risk of bias                                                 \\
                            &                                                          & NER and Text   Classification & NER                                                    \\
                            &                                                          & Relation Extraction                               & Entity   Linking \\                                                      
\bottomrule
\end{tabular}
\end{table}

==> tables/SLR_Methodologies.tex <==
\begin{table}[]
\centering
\footnotesize
\caption{Strategies adopted in the previous eight SLR surveys. Y = Yes , N=No, S=Source, M=Methodology.\label{tab:slr_methodologies}}
\begin{tabular}{l|p{7cm}|c|c|c|c|c|c|c}
\toprule
\textbf{\#} & \textbf{Survey Paper Title} & \Rot{\textbf{Web Search (S)}} & \Rot{\textbf{SR Toolbox (S)}} & \Rot{\textbf{Previous Studies (S)}} & \Rot{\textbf{Interviews (S)}}& \Rot{\textbf{Search Strategy (M)}} & \Rot{\textbf{Snowballing (M)}}  & \textbf{Ref.} \\
\midrule
1  &  Tools to support systematic reviews in software engineering: a feature analysis    & \cellcolor[HTML]{FFC7C4}N    & \cellcolor[HTML]{FFC7C4}N    & \cellcolor[HTML]{C6EFCE}Y   & \cellcolor[HTML]{FFC7C4}N& \cellcolor[HTML]{FFC7C4}N  & \cellcolor[HTML]{FFC7C4}N    & \cite{marshall2014tools}    \\ \hline
2  & Online tools supporting the conduct and reporting of systematic reviews and systematic maps: a case study on cadima and review of existing tools    & \cellcolor[HTML]{C6EFCE}Y    & \cellcolor[HTML]{C6EFCE}Y    & \cellcolor[HTML]{C6EFCE}Y   & \cellcolor[HTML]{FFC7C4}N& \cellcolor[HTML]{C6EFCE}Y  & \cellcolor[HTML]{C6EFCE}Y    & \cite{kohl2018online}       \\ \hline
3  &  Software tools for literature screening in systematic reviews in biomedical research    & \cellcolor[HTML]{FFC7C4}N    & \cellcolor[HTML]{C6EFCE}Y    & \cellcolor[HTML]{FFC7C4}N   & \cellcolor[HTML]{C6EFCE}Y& \cellcolor[HTML]{FFC7C4}N  & \cellcolor[HTML]{FFC7C4}N    & \cite{van2019software}      \\ \hline
4  &   Software tools to support title and abstract screening for systematic reviews in healthcare: an evaluation   & \cellcolor[HTML]{C6EFCE}Y    & \cellcolor[HTML]{C6EFCE}Y    & \cellcolor[HTML]{C6EFCE}Y   & \cellcolor[HTML]{FFC7C4}N& \cellcolor[HTML]{FFC7C4}N  & \cellcolor[HTML]{FFC7C4}N    & \cite{harrison2020software} \\ \hline
5  &  Web-Based Software Tools for Systematic Literature Review in Medicine: Systematic Search and Feature Analysis    & \cellcolor[HTML]{C6EFCE}Y    & \cellcolor[HTML]{C6EFCE}Y    & \cellcolor[HTML]{C6EFCE}Y   & \cellcolor[HTML]{FFC7C4}N& \cellcolor[HTML]{FFC7C4}N  & \cellcolor[HTML]{FFC7C4}N    & \cite{cowie2022web}         \\ \hline
6  &  “hasta la vista, baby”–will machine learning terminate human literature reviews in entrepreneurship?    & \cellcolor[HTML]{C6EFCE}Y    & \cellcolor[HTML]{C6EFCE}Y    & \cellcolor[HTML]{C6EFCE}Y   & \cellcolor[HTML]{FFC7C4}N& \cellcolor[HTML]{FFC7C4}N  & \cellcolor[HTML]{FFC7C4}N    & \cite{robledo2023vista}     \\ \hline
7  &  Reducing literature screening workload with machine learning.    & \cellcolor[HTML]{FFC7C4}N    & \cellcolor[HTML]{FFC7C4}N    & \cellcolor[HTML]{C6EFCE}Y   & \cellcolor[HTML]{FFC7C4}N& \cellcolor[HTML]{C6EFCE}Y  & \cellcolor[HTML]{C6EFCE}Y    & \cite{burgard2023reducing}  \\ \hline
8  &   Artificial intelligence to automate the systematic review of scientific literature.    & \cellcolor[HTML]{FFC7C4}N    & \cellcolor[HTML]{FFC7C4}N    & \cellcolor[HTML]{FFC7C4}N   & \cellcolor[HTML]{FFC7C4}N& \cellcolor[HTML]{C6EFCE}Y  & \cellcolor[HTML]{C6EFCE}Y    & \cite{de2023artificial}     \\ 
  
\bottomrule
\end{tabular}
% \begin{tablenotes}[para,flushleft]
%      \textbf{Note:} Y = Yes , N=No, S=Source, M=Methodology.
% \end{tablenotes}

\end{table}




% \begin{table}[]
% \centering
% \footnotesize
% \caption{Methodologies implemented in previous surveys about SLRs. Y = Yes , N=No, S=Source, M=Methodology.\label{tab:slr_methodologies}}
% \begin{tabular}{l|c|c|c|c|c|c|c}
% \toprule
% \textbf{\#} & \Rot{\textbf{Reference}} & \Rot{\textbf{Web Search (S)}} & \Rot{\textbf{SR Toolbox (S)}} & \Rot{\textbf{Previous Studies (S)}} & \Rot{\textbf{Other Sources (S)}}& \Rot{\textbf{Search Strategy (M)}} & \Rot{\textbf{Snowballing(M)}}   \\
% \midrule
% 1 & \cite{marshall2014tools}  & N & N & Y & N & N & N\\
% 2 & \cite{kohl2018online}  & Y & Y & Y & N& Y & Y\\
% 3 & \cite{van2019software}  & N & Y & N & Y & N & N \\
% 4 & \cite{harrison2020software}  & Y & Y & Y & N & N & N \\
% 5 & \cite{cowie2022web}  & Y & Y & Y & N & N & N \\
% 6 & \cite{robledo2023vista}  & Y & Y & Y & N & N & N \\
% 7 & \cite{burgard2023reducing}  & N & N & Y & N & Y & Y \\
% 8 & \cite{de2023artificial}  & N & N & N & N & Y & Y \\
  
% \bottomrule
% \end{tabular}
% % \begin{tablenotes}[para,flushleft]
% %      \textbf{Note:} Y = Yes , N=No, S=Source, M=Methodology.
% % \end{tablenotes}

% \end{table}



==> tables/TableA1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[]
  \caption{Tools for the screening phase described according to the AI features}
    \label{tab:tools_described_ai_features_screening}
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l}
Tool                      & Research Field & SLR Task                                                                                                                                                                                                                                                                                                              & Human   Interaction                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               & Approach                                                                                                                                                                                                                                                                                                                                                                                                                                            & Text   Representation                                                                                                                                                                                 & Input                                                                                                                                                                                                 & Output                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               & Minimum   Requirement                                                                                                                                                                & Model Execution                                                                                                                                                      & Pre-screening   Support                                                                                                                                                                                                                                                                                                                                                                                                                                                                       & Post-Screening   Support                                  \\
Abstrackr                 & Any            & Classification   of relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML   classifier (Active Learning) based on SMV applying constrained weightspace.                                                                                                                                                                                                                                                                                                                                                                    & bag   of words: Information not available.                                                                                                                                                            & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:   Pre classification of papers based on inclusion probability (Not   Available).\\      Range: Information not available.\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}Relevant   papers: Information not available.\\      Irrelevant papers: Information not available.\end{tabular}                                           & Synchronous:   the model runs in the background.                                                                                                                     & Keywords   search: It searches by    keywords that could be color by level of relevance.                                                                                                                                                                                                                                                                                                                                                                                                      & None                                                      \\
ASReview                  & Any            & Classification   of relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML   classifier (Active Learning) based on Naive Bayes(default), SMV , logistic   regression,  RandoM Forest or Simple   NN.                                                                                                                                                                                                                                                                                                                        & \begin{tabular}[c]{@{}l@{}}bag   of words: Information not available.\\      embeddings:sentence BERT, doc2vec.\end{tabular}                                                                          & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability ( likelihood of   relevance).\\      Range: 0-1.\\      Threshold: For values greater than 0.5 the papers are marked as relevant.\end{tabular}                                                                                                                                                                                                                                                                         & \begin{tabular}[c]{@{}l@{}}Relevant   papers: 1.\\      Irrelevant papers:1.\end{tabular}                                                                                            & Synchronous:   the model runs in the background.                                                                                                                     & Keywords search: Basic search trough keywords                                                                                                                                                                                                                                                                                                                                                                                                                                                 & None                                                      \\
Colandr                   & Any            & \begin{tabular}[c]{@{}l@{}}Task 1     Classification of relevant papers given a set of   seed papers.\\      Task 2     Identification of the category attributed to the paper by the user\end{tabular}                                                                                                               & \begin{tabular}[c]{@{}l@{}}Task 1      The user has to rank papers as   relevant and irrelevant.\\      Task 2     The user has to assigned categories(tags) to the papers.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & \begin{tabular}[c]{@{}l@{}}Task 1     Similarity-based method: Identifies co-occurrences of words around the   keywords selected by the user (Active Learning).\\      Task 2     2.1 NER for  Locations (Active   Learning).\\      2.2 ML classifier for other tags based on logistic regression (Active   Learning).\end{tabular}                                                                                                                & \begin{tabular}[c]{@{}l@{}}Task 1     embeddings: Word2vec.\\      Task 2     2.1 Information not available.\\      2.2 embeddings: Glove\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}Task 1\\      The title and    abstract of the paper in the accepted format.\\      Task 2\\      Full-text papers in PDF.\end{tabular}                                    & \begin{tabular}[c]{@{}l@{}}Task 1     Name:Pre classification of papers based on inclusion probability   (relevance).\\      Range: Information not available.\\      Threshold: Information not available.\\      Task 2     Name:Listing of sentences that best predicts the label (confident).\\      Range: High, Medium, Low.\\      Threshold: Information not available.\end{tabular}                                                                                                                         & \begin{tabular}[c]{@{}l@{}}Task 1     Relevant papers: 10.\\      Irrelevant papers:10.\\      Task 2     Minimum 50 papers.\end{tabular}                                            & \begin{tabular}[c]{@{}l@{}}Task 1     Synchronous: the model runs in the background.\\      Task 2     Synchronous: the model runs in the background.\end{tabular}   & Keywords search: It searches by  keywords that could be color by level of   relevance.                                                                                                                                                                                                                                                                                                                                                                                                        & None                                                      \\
Covidence                 & Any            & \begin{tabular}[c]{@{}l@{}}Task 1     Classification of relevant papers given a set of seed papers.\\      Task 2     Identification of biomedical studies(RCTs) based on a pre-built   classification model.\end{tabular}                                                                                            & \begin{tabular}[c]{@{}l@{}}Task 1      The user has to rank papers as   relevant and irrelevant.\\      Task 2     No user interaction.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              & \begin{tabular}[c]{@{}l@{}}Task 1     ML classifier (Active Learning) based on two ensembles SVM.\\      Task 2     ML classifier (Superivised Learning) bassed on SVM (RCT classifier).\end{tabular}                                                                                                                                                                                                                                               & \begin{tabular}[c]{@{}l@{}}Task 1     bag of words: ngrams.\\      Task 2      bag of words: ngrams.\end{tabular}                                                                                     & \begin{tabular}[c]{@{}l@{}}Task 1     The title and  abstract of the paper   in the accepted format.\\      Task 2\\      The title and    abstract of the paper in the accepted format.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Task 1     Name:Pre classification of papers based on inclusion probability (relevancy   prediction).\\      Range: Information not available.\\      Threshold: Information not available.\\      Task 2     Name:Pre classification of papers based on inclusion probability (not   Available)\\      Range: (0-1){[}Possible RCT, Not RCT{]}\\      Threshold: For values greater than 0.24 the papers are marked as Possible   RCT.\end{tabular}                                      & \begin{tabular}[c]{@{}l@{}}Task 1     Relevant papers: 2.\\      Irrelevant papers: 2.\\      Task 2     Not Applicable.\end{tabular}                                                & Information   not available.                                                                                                                                         & Keywords search: Basic search trough keywords                                                                                                                                                                                                                                                                                                                                                                                                                                                 & None                                                      \\
DistillerSR               & Any            & Classification   of relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML   classifiers (Active Learning) based on SVM or Naive Bayes.                                                                                                                                                                                                                                                                                                                                                                                     & bag   of words: Information not available.                                                                                                                                                            & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Naive Bayes     Name:Pre classification of papers based on inclusion probability   (prediction score).\\      Range: 0-1\\      Threshold:  For values greater or   equal than 0.5 the papers are likely to marked as relevant.\\      SVM     Name:Pre classification of papers based on binary classification.\\      Range: (0-1) {[}Include, Exclude, or Cannot Decide{]}.\\      Threshold: Information not available.\end{tabular}                                                  & \begin{tabular}[c]{@{}l@{}}Relevant   papers: 10.\\      Irrelevant papers:40.\end{tabular}                                                                                          & Information not   available.                                                                                                                                         & Keywords search: Basic search trough keywords                                                                                                                                                                                                                                                                                                                                                                                                                                                 & None                                                      \\
EPPI-Reviewer             & Any            & \begin{tabular}[c]{@{}l@{}}Task 1\\      Classification of relevant papers given a set of   seed papers.\\      Task 2\\      Identification of biomedical studies (RCTs,   Systematic Reviews,  Economic   Evaluations,  COVID-19 categories,  long COVID) based on a pre-built   classification model.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Task 1     The user has to rank papers as relevant and irrelevant.\\      Task 2     No user interaction.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}Task 1     ML classifier (Active Learning) based on SVM. \\      Task 2     ML classifier (Superivised Learning) based on SVM for 2.1 and for the   others the information is not available.\\           2.1 Cochrane RCT.\\           2.2  Origina RCT.\\           2.3 Systematic Review.\\           2.4 Economic Evaluations. \\           2.5 COVID-19 categories.\\          2.6 Identify Long COVID.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Task 1     bag of words: ngrams.\\      Task 2     The Cochrane RCT classifer uses bag of words. For the other approaches the   information is not available.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Task 1     The title and  abstract of the paper   in the accepted format.\\      Task 2     The title and  abstract of the paper   in the accepted format.\end{tabular}    & \begin{tabular}[c]{@{}l@{}}Task 1     Name:Pre classification of papers based on   inclusion probability (probability score).\\      Range: 0-100\\      Threshold: Information not available.\\      Task 2\\      Case: Cochrane RCT\\                Name:Pre classification of   papers based on inclusion probability (not Available)\\                Range: (0-1){[}Possible RCT,   Not RCT{]}\\                Threshold: For values   greater than 0.24 the papers are marked as Possible RCT.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Task 1     Relevant papers: 5.\\      Irrelevant papers: Information not available.\\      Task 2     Not Applicable\end{tabular}                         & \begin{tabular}[c]{@{}l@{}}Task 1     Synchronous: the model runs in the background.\\      Task 2     Synchronous: the model runs in the background.\end{tabular}   & \begin{tabular}[c]{@{}l@{}}Keywords   search: It searches by    keywords that could be highlighted;\\      Tags: It searches   by  terms or tags assigned after   reading the paper.\end{tabular}                                                                                                                                                                                                                                                                                             & None                                                      \\
FAST2                     & Any            & Classification of   relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML classifier (Active   Learning) based on SVM.                                                                                                                                                                                                                                                                                                                                                                                                     & bag   of words: Information not available.                                                                                                                                                            & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability (decision   score).\\      Range: 0-1\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                                                                                                                                                        & \begin{tabular}[c]{@{}l@{}}Relevant   papers: Information not available.\\      Irrelevant papers: Information not available.\end{tabular}                                           & Synchronous: the   model runs in the background.                                                                                                                     & None                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & None                                                      \\
Iris.ai                   & Any            & Clustering of   Abstracts                                                                                                                                                                                                                                                                                             & \begin{tabular}[c]{@{}l@{}}1.   Exploratory search: When the researcher is novice or exploring a new   field.\\           1.1 The user has to  provide a seed idea (300-500 words) or a   title or abstract of a paper.\\           1.2  The user has to select the relevant papers   from the visual map manually or using the search filter. In the latter he can   narrow down the results based on topics or concepts using the analyze   tool.\\      \\      2. Advanced search: When the researcher has expertise on the topic.\\           2.1 The user has to select a   dataset, it could be retrieved from a database or his own records.\\           2.2 The user can cluster the   results using the search filter option which will allow him to  apply the    analyze tool and/or the context filter.\\           2.3 The user has to select the   relavant papers.\\           2.4  The user can repeat steps 2.2 and 2.3  until he considers appropriate to   stop.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Similarity-based   method: Matches the fingerprint of the text or abstract with the fingerprints   of the papers of the databases CORE, PubMed,    US Patent or CORDIS.(Unsupervised Learning).\\      \\      The fingerprint is a vector representation of the most meaningful words   and  their synonyms of the text or   abstract which has a unique numerical value.\end{tabular}                                  & embeddings:   Information not available.                                                                                                                                                              & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability (relevance   score).\\      Range: (0-1){[}Percentage{]}\\      Threshold: 40\%-90\%\end{tabular}                                                                                                                                                                                                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Relevant   papers: Not Applicable.\\      Irrelevant papers: Not Applicable.\end{tabular}                                                                 & Synchronous: the   model runs in the background.                                                                                                                     & \begin{tabular}[c]{@{}l@{}}Keywords   search: Basic search trough keywords;\\      Topic Groups: from a   global topic (what topics do these articles fall within from an overall   scientific level) as well as a specific topic (within this reading list, what topics do the articles fall within) based on   visual maps.\end{tabular}                                                                                                                                                    & Abstractive   summarisation based on the selected papers. \\
LitSuggest                & Biomedicine    & Classification   of relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML   classifier ( Active Learning) based on logistic regression.                                                                                                                                                                                                                                                                                                                                                                                    & bag   of words: Information not available.                                                                                                                                                            & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability (relevance   prediction).\\      Range: 0-1.\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}Relevant   papers: Information not available.\\      Irrelevant papers: Information not available.\end{tabular}                                           & Synchronous:   the model runs in the background.                                                                                                                     & None                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & None                                                      \\
Nested   Knowledge        & Any            & Classification   of relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML   classifier (Active Learning) which is unkown.                                                                                                                                                                                                                                                                                                                                                                                                  & Information not   available.                                                                                                                                                                          & The   title and  abstractof the paper in the   accepted format.                                                                                                                                       & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability (inclusion   prediction).\\      Range: Information not available.\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                                                                                                                           & \begin{tabular}[c]{@{}l@{}}Relevant   papers: Information not available.\\      Irrelevant papers: Information not available.\end{tabular}                                           & Information not   available.                                                                                                                                         & \begin{tabular}[c]{@{}l@{}}Keywords   search: Basic search trough keywords;\\      PICO identification: Highlights   the parts of a PICO  question in the   abstract;\end{tabular}                                                                                                                                                                                                                                                                                                            & Ontology based on the   user classification.              \\
PICOPortal                & Any            & \begin{tabular}[c]{@{}l@{}}Task 1     Classification of relevant papers given a set of seed papers.\\      Task 2     Identification of biomedical studies(RCTs) based on a pre-built   classification model.\end{tabular}                                                                                            & \begin{tabular}[c]{@{}l@{}}Task 1     The user has to rank papers as relevant and   irrelevant.\\      Task 2\\      No user interaction.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            & \begin{tabular}[c]{@{}l@{}}Task 1     ML classifier (Active Learning) based on SVM.\\      Task 2     ML classifier (Superivised Learning) based voting system implementing   decision tree or deep learning.\end{tabular}                                                                                                                                                                                                                          & \begin{tabular}[c]{@{}l@{}}Task 1     Information not available.\\      Task 2     embeddings: BioBERT.\end{tabular}                                                                                  & \begin{tabular}[c]{@{}l@{}}Task 1     The title and  abstract of the paper   in the accepted format.\\      Task  2     The title and  abstract of the paper   in the accepted format.\end{tabular}   & \begin{tabular}[c]{@{}l@{}}Task 1     NamePre classification of papers based on inclusion probability (not   Available)\\      Range: Information not available.\\      Threshold: Information not available.\\      Task 2     Name:Pre classification of papers based on inclusion probability (not   Available)\\      Range: (0-1){[}Possible RCT, Not RCT{]}.\\      Threshold:  Information not   available.\end{tabular}                                                                                      & \begin{tabular}[c]{@{}l@{}}Task 1     Relevant papers: Information not available.\\      Irrelevant papers:Information not available.\\      Task 2     Not Applicable.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Task 1     Synchronous: the model runs in the background.     Task 2\\      Synchronous: the model runs in the   background.\end{tabular} & PICO identification: Highlights the   parts of a PICO  question in the   abstract.                                                                                                                                                                                                                                                                                                                                                                                                            & None                                                      \\
pitts.ai                  & Biomedicine    & Identification   of biomedical studies(RCTs) based on a pre-built classification model.                                                                                                                                                                                                                               & No   user interaction.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            & ML classifier   (Superivised Learning) based on SVM.                                                                                                                                                                                                                                                                                                                                                                                                & embeddings:SciBERT                                                                                                                                                                                    & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre classification of papers based on inclusion   probability (prediction probability).     Range: 0-1.\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                                                                                                                                                    & \begin{tabular}[c]{@{}l@{}}Relevant   papers:  Not Applicable.\\      Irrelevant papers:  Not Applicable.\end{tabular}                                                               & Synchronous: the   model runs in the background.                                                                                                                     & None                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & None                                                      \\
Rayyan                    & Any            & Classification   of relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML   classifier (Active Learning) based on SVM.                                                                                                                                                                                                                                                                                                                                                                                                     & bag   of words:ngrams                                                                                                                                                                                 & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability(score   probability)\\      Range: A 5 star scheme, the closer to 5 the    paper be consider as relevant\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                                                                                     & \begin{tabular}[c]{@{}l@{}}Relevant   papers: 5.\\      Irrelevant papers:5.\end{tabular}                                                                                            & Synchronous:   the model runs in the background.                                                                                                                     & \begin{tabular}[c]{@{}l@{}}Keywords   search: It searches by    keywords that could be highlighted;\\      Other searches: It   searches by author or publication year;\\      Boolean Operator: It searches by the combination of boolean operators(AND, OR,   NOT) with keywords.\end{tabular}                                                                                                                                                                                              & None                                                      \\
Research   Screener       & Any            & Classification   of relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML   classifier (Active Learning) based on unkown algorithm.                                                                                                                                                                                                                                                                                                                                                                                        & embeddings:   paragraph embedding                                                                                                                                                                     & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability(inclusion   probability)\\      Range: Information not available.\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                                                                                                                            & \begin{tabular}[c]{@{}l@{}}Relevant   papers: 1.\\      Irrelevant papers: Information not available.\end{tabular}                                                                   & Synchronous:   the model runs in the background.                                                                                                                     & None                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & None                                                      \\
RobotAnalyst              & Any            & Classification   of relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML   classifier (Active Learning) based on SVM.                                                                                                                                                                                                                                                                                                                                                                                                     & bag   of words: Information not available.                                                                                                                                                            & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability(inclusion   confidence)\\      Range: 0-1\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                                                                                                                                                    & Relevant   papers: Information not available.     Irrelevant papers: Information not available.                                                                                      & Synchronous:   the model runs in the background.                                                                                                                     & Topic   modelling: It assigned    a topic to a paper based on the    most recurrent terms which    could be shared by other papers; clustering: groups paper on the most common terms that are not overlap; Keywords search: searches by   keywords; term search: searches   by terms(noun phrases)  extracted from   the title and abstract; Other criterias: Document id, Publication Year, Author, Type of Publication,   Journal, Notes, Time of screening decision,    retrieval method; & None                                                      \\
RobotReviewer/RobotSearch & Biomedicine    & Identification of biomedical studies(RCTs)   based on a pre-built classification model.                                                                                                                                                                                                                               & No user interaction.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              & ML classifier (Active   Learning) based on SVM.                                                                                                                                                                                                                                                                                                                                                                                                     & embeddings:SciBERT                                                                                                                                                                                    & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability(prediction   probability).\\      Range: 0-1.\\      Threshold: Not Available.\end{tabular}                                                                                                                                                                                                                                                                                                                            & \begin{tabular}[c]{@{}l@{}}Relevant   papers: Not Applicable.\\      Irrelevant papers:Not Applicable.\end{tabular}                                                                  & Information not   available.                                                                                                                                         & PICO model:  It colour the  different PICO elements.                                                                                                                                                                                                                                                                                                                                                                                                                                          & Pending                                                   \\
SWIFT-Active   Screener   & Any            & Classification   of relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML   classifier (Active Learning) based on log-linear.                                                                                                                                                                                                                                                                                                                                                                                              & bag   of words: Information not available.                                                                                                                                                            & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability(inclusion   rate).\\      Range: 0-1.\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                                                                                                                                                        & \begin{tabular}[c]{@{}l@{}}Relevant   papers: 1.\\      Irrelevant papers:1.\end{tabular}                                                                                            & Asynchronous:   The model updates every  30 papers.   There must be a gap of 2 minutes between the last model built and the current   model built.                   & Keywords search: Basic search trough   keywords                                                                                                                                                                                                                                                                                                                                                                                                                                               & None                                                      \\
SWIFT-Review              & Biomedicine    & Classification   of relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML   classifier (Active Learning) based on log-linear.                                                                                                                                                                                                                                                                                                                                                                                              & bag   of words: Information not available.                                                                                                                                                            & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability(priority  ranking).\\      Range: 0-1.\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                                                                                                                                                       & \begin{tabular}[c]{@{}l@{}}Relevant   papers: 1.\\      Irrelevant papers:1.\end{tabular}                                                                                            & Synchronous:   the model runs in the background.                                                                                                                     & \begin{tabular}[c]{@{}l@{}}Keywords   search: Basic search trough keywords.     \\      Topic modelling: It assigned  a topic to a paper based on the  most recurrent terms which  could be shared by other papers; Keywor   search: searches by keywords or tags;\end{tabular}                                                                                                                                                                                                               & None                                                      \\
SysRev.com                & Any            & Classification   of relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML   classifier (Active Learning) based on a customized architecture similar to   cross attention.                                                                                                                                                                                                                                                                                                                                                  & Information not   available.                                                                                                                                                                          & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability(prediction   probability).\\      Range: Information not available.\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                                                                                                                          & \begin{tabular}[c]{@{}l@{}}Relevant   papers: 30.\\      Irrelevant papers: 30.\end{tabular}                                                                                         & Asynchronous: The   model updates nightly.                                                                                                                           & None                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & None                                                     
\end{tabular}
\end{table}
\begin{table}[]
\begin{tabular}{llllllllllll}
Tool                      & Research Field & SLR Task                                                                                                                                                                                                                                                                                                              & Human   Interaction                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               & Approach                                                                                                                                                                                                                                                                                                                                                                                                                                            & Text   Representation                                                                                                                                                                                 & Input                                                                                                                                                                                                 & Output                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               & Minimum   Requirement                                                                                                                                                                & Model Execution                                                                                                                                                      & Pre-screening   Support                                                                                                                                                                                                                                                                                                                                                                                                                                                                       & Post-Screening   Support                                  \\
Abstrackr                 & Any            & Classification   of relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML   classifier (Active Learning) based on SMV applying constrained weightspace.                                                                                                                                                                                                                                                                                                                                                                    & bag   of words: Information not available.                                                                                                                                                            & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:   Pre classification of papers based on inclusion probability (Not   Available).\\      Range: Information not available.\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}Relevant   papers: Information not available.\\      Irrelevant papers: Information not available.\end{tabular}                                           & Synchronous:   the model runs in the background.                                                                                                                     & Keywords   search: It searches by    keywords that could be color by level of relevance.                                                                                                                                                                                                                                                                                                                                                                                                      & None                                                      \\
ASReview                  & Any            & Classification   of relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML   classifier (Active Learning) based on Naive Bayes(default), SMV , logistic   regression,  RandoM Forest or Simple   NN.                                                                                                                                                                                                                                                                                                                        & \begin{tabular}[c]{@{}l@{}}bag   of words: Information not available.\\      embeddings:sentence BERT, doc2vec.\end{tabular}                                                                          & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability ( likelihood of   relevance).\\      Range: 0-1.\\      Threshold: For values greater than 0.5 the papers are marked as relevant.\end{tabular}                                                                                                                                                                                                                                                                         & \begin{tabular}[c]{@{}l@{}}Relevant   papers: 1.\\      Irrelevant papers:1.\end{tabular}                                                                                            & Synchronous:   the model runs in the background.                                                                                                                     & Keywords search: Basic search trough keywords                                                                                                                                                                                                                                                                                                                                                                                                                                                 & None                                                      \\
Colandr                   & Any            & \begin{tabular}[c]{@{}l@{}}Task 1     Classification of relevant papers given a set of   seed papers.\\      Task 2     Identification of the category attributed to the paper by the user\end{tabular}                                                                                                               & \begin{tabular}[c]{@{}l@{}}Task 1      The user has to rank papers as   relevant and irrelevant.\\      Task 2     The user has to assigned categories(tags) to the papers.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & \begin{tabular}[c]{@{}l@{}}Task 1     Similarity-based method: Identifies co-occurrences of words around the   keywords selected by the user (Active Learning).\\      Task 2     2.1 NER for  Locations (Active   Learning).\\      2.2 ML classifier for other tags based on logistic regression (Active   Learning).\end{tabular}                                                                                                                & \begin{tabular}[c]{@{}l@{}}Task 1     embeddings: Word2vec.\\      Task 2     2.1 Information not available.\\      2.2 embeddings: Glove\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}Task 1\\      The title and    abstract of the paper in the accepted format.\\      Task 2\\      Full-text papers in PDF.\end{tabular}                                    & \begin{tabular}[c]{@{}l@{}}Task 1     Name:Pre classification of papers based on inclusion probability   (relevance).\\      Range: Information not available.\\      Threshold: Information not available.\\      Task 2     Name:Listing of sentences that best predicts the label (confident).\\      Range: High, Medium, Low.\\      Threshold: Information not available.\end{tabular}                                                                                                                         & \begin{tabular}[c]{@{}l@{}}Task 1     Relevant papers: 10.\\      Irrelevant papers:10.\\      Task 2     Minimum 50 papers.\end{tabular}                                            & \begin{tabular}[c]{@{}l@{}}Task 1     Synchronous: the model runs in the background.\\      Task 2     Synchronous: the model runs in the background.\end{tabular}   & Keywords search: It searches by  keywords that could be color by level of   relevance.                                                                                                                                                                                                                                                                                                                                                                                                        & None                                                      \\
Covidence                 & Any            & \begin{tabular}[c]{@{}l@{}}Task 1     Classification of relevant papers given a set of seed papers.\\      Task 2     Identification of biomedical studies(RCTs) based on a pre-built   classification model.\end{tabular}                                                                                            & \begin{tabular}[c]{@{}l@{}}Task 1      The user has to rank papers as   relevant and irrelevant.\\      Task 2     No user interaction.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              & \begin{tabular}[c]{@{}l@{}}Task 1     ML classifier (Active Learning) based on two ensembles SVM.\\      Task 2     ML classifier (Superivised Learning) bassed on SVM (RCT classifier).\end{tabular}                                                                                                                                                                                                                                               & \begin{tabular}[c]{@{}l@{}}Task 1     bag of words: ngrams.\\      Task 2      bag of words: ngrams.\end{tabular}                                                                                     & \begin{tabular}[c]{@{}l@{}}Task 1     The title and  abstract of the paper   in the accepted format.\\      Task 2\\      The title and    abstract of the paper in the accepted format.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Task 1     Name:Pre classification of papers based on inclusion probability (relevancy   prediction).\\      Range: Information not available.\\      Threshold: Information not available.\\      Task 2     Name:Pre classification of papers based on inclusion probability (not   Available)\\      Range: (0-1){[}Possible RCT, Not RCT{]}\\      Threshold: For values greater than 0.24 the papers are marked as Possible   RCT.\end{tabular}                                      & \begin{tabular}[c]{@{}l@{}}Task 1     Relevant papers: 2.\\      Irrelevant papers: 2.\\      Task 2     Not Applicable.\end{tabular}                                                & Information   not available.                                                                                                                                         & Keywords search: Basic search trough keywords                                                                                                                                                                                                                                                                                                                                                                                                                                                 & None                                                      \\
DistillerSR               & Any            & Classification   of relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML   classifiers (Active Learning) based on SVM or Naive Bayes.                                                                                                                                                                                                                                                                                                                                                                                     & bag   of words: Information not available.                                                                                                                                                            & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Naive Bayes     Name:Pre classification of papers based on inclusion probability   (prediction score).\\      Range: 0-1\\      Threshold:  For values greater or   equal than 0.5 the papers are likely to marked as relevant.\\      SVM     Name:Pre classification of papers based on binary classification.\\      Range: (0-1) {[}Include, Exclude, or Cannot Decide{]}.\\      Threshold: Information not available.\end{tabular}                                                  & \begin{tabular}[c]{@{}l@{}}Relevant   papers: 10.\\      Irrelevant papers:40.\end{tabular}                                                                                          & Information not   available.                                                                                                                                         & Keywords search: Basic search trough keywords                                                                                                                                                                                                                                                                                                                                                                                                                                                 & None                                                      \\
EPPI-Reviewer             & Any            & \begin{tabular}[c]{@{}l@{}}Task 1\\      Classification of relevant papers given a set of   seed papers.\\      Task 2\\      Identification of biomedical studies (RCTs,   Systematic Reviews,  Economic   Evaluations,  COVID-19 categories,  long COVID) based on a pre-built   classification model.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Task 1     The user has to rank papers as relevant and irrelevant.\\      Task 2     No user interaction.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}Task 1     ML classifier (Active Learning) based on SVM. \\      Task 2     ML classifier (Superivised Learning) based on SVM for 2.1 and for the   others the information is not available.\\           2.1 Cochrane RCT.\\           2.2  Origina RCT.\\           2.3 Systematic Review.\\           2.4 Economic Evaluations. \\           2.5 COVID-19 categories.\\          2.6 Identify Long COVID.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Task 1     bag of words: ngrams.\\      Task 2     The Cochrane RCT classifer uses bag of words. For the other approaches the   information is not available.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Task 1     The title and  abstract of the paper   in the accepted format.\\      Task 2     The title and  abstract of the paper   in the accepted format.\end{tabular}    & \begin{tabular}[c]{@{}l@{}}Task 1     Name:Pre classification of papers based on   inclusion probability (probability score).\\      Range: 0-100\\      Threshold: Information not available.\\      Task 2\\      Case: Cochrane RCT\\                Name:Pre classification of   papers based on inclusion probability (not Available)\\                Range: (0-1){[}Possible RCT,   Not RCT{]}\\                Threshold: For values   greater than 0.24 the papers are marked as Possible RCT.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Task 1     Relevant papers: 5.\\      Irrelevant papers: Information not available.\\      Task 2     Not Applicable\end{tabular}                         & \begin{tabular}[c]{@{}l@{}}Task 1     Synchronous: the model runs in the background.\\      Task 2     Synchronous: the model runs in the background.\end{tabular}   & \begin{tabular}[c]{@{}l@{}}Keywords   search: It searches by    keywords that could be highlighted;\\      Tags: It searches   by  terms or tags assigned after   reading the paper.\end{tabular}                                                                                                                                                                                                                                                                                             & None                                                      \\
FAST2                     & Any            & Classification of   relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML classifier (Active   Learning) based on SVM.                                                                                                                                                                                                                                                                                                                                                                                                     & bag   of words: Information not available.                                                                                                                                                            & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability (decision   score).\\      Range: 0-1\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                                                                                                                                                        & \begin{tabular}[c]{@{}l@{}}Relevant   papers: Information not available.\\      Irrelevant papers: Information not available.\end{tabular}                                           & Synchronous: the   model runs in the background.                                                                                                                     & None                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & None                                                      \\
Iris.ai                   & Any            & Clustering of   Abstracts                                                                                                                                                                                                                                                                                             & \begin{tabular}[c]{@{}l@{}}1.   Exploratory search: When the researcher is novice or exploring a new   field.\\           1.1 The user has to  provide a seed idea (300-500 words) or a   title or abstract of a paper.\\           1.2  The user has to select the relevant papers   from the visual map manually or using the search filter. In the latter he can   narrow down the results based on topics or concepts using the analyze   tool.\\      \\      2. Advanced search: When the researcher has expertise on the topic.\\           2.1 The user has to select a   dataset, it could be retrieved from a database or his own records.\\           2.2 The user can cluster the   results using the search filter option which will allow him to  apply the    analyze tool and/or the context filter.\\           2.3 The user has to select the   relavant papers.\\           2.4  The user can repeat steps 2.2 and 2.3  until he considers appropriate to   stop.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Similarity-based   method: Matches the fingerprint of the text or abstract with the fingerprints   of the papers of the databases CORE, PubMed,    US Patent or CORDIS.(Unsupervised Learning).\\      \\      The fingerprint is a vector representation of the most meaningful words   and  their synonyms of the text or   abstract which has a unique numerical value.\end{tabular}                                  & embeddings:   Information not available.                                                                                                                                                              & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability (relevance   score).\\      Range: (0-1){[}Percentage{]}\\      Threshold: 40\%-90\%\end{tabular}                                                                                                                                                                                                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Relevant   papers: Not Applicable.\\      Irrelevant papers: Not Applicable.\end{tabular}                                                                 & Synchronous: the   model runs in the background.                                                                                                                     & \begin{tabular}[c]{@{}l@{}}Keywords   search: Basic search trough keywords;\\      Topic Groups: from a   global topic (what topics do these articles fall within from an overall   scientific level) as well as a specific topic (within this reading list, what topics do the articles fall within) based on   visual maps.\end{tabular}                                                                                                                                                    & Abstractive   summarisation based on the selected papers. \\
LitSuggest                & Biomedicine    & Classification   of relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML   classifier ( Active Learning) based on logistic regression.                                                                                                                                                                                                                                                                                                                                                                                    & bag   of words: Information not available.                                                                                                                                                            & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability (relevance   prediction).\\      Range: 0-1.\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}Relevant   papers: Information not available.\\      Irrelevant papers: Information not available.\end{tabular}                                           & Synchronous:   the model runs in the background.                                                                                                                     & None                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & None                                                      \\
Nested   Knowledge        & Any            & Classification   of relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML   classifier (Active Learning) which is unkown.                                                                                                                                                                                                                                                                                                                                                                                                  & Information not   available.                                                                                                                                                                          & The   title and  abstractof the paper in the   accepted format.                                                                                                                                       & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability (inclusion   prediction).\\      Range: Information not available.\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                                                                                                                           & \begin{tabular}[c]{@{}l@{}}Relevant   papers: Information not available.\\      Irrelevant papers: Information not available.\end{tabular}                                           & Information not   available.                                                                                                                                         & \begin{tabular}[c]{@{}l@{}}Keywords   search: Basic search trough keywords;\\      PICO identification: Highlights   the parts of a PICO  question in the   abstract;\end{tabular}                                                                                                                                                                                                                                                                                                            & Ontology based on the   user classification.              \\
PICOPortal                & Any            & \begin{tabular}[c]{@{}l@{}}Task 1     Classification of relevant papers given a set of seed papers.\\      Task 2     Identification of biomedical studies(RCTs) based on a pre-built   classification model.\end{tabular}                                                                                            & \begin{tabular}[c]{@{}l@{}}Task 1     The user has to rank papers as relevant and   irrelevant.\\      Task 2\\      No user interaction.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            & \begin{tabular}[c]{@{}l@{}}Task 1     ML classifier (Active Learning) based on SVM.\\      Task 2     ML classifier (Superivised Learning) based voting system implementing   decision tree or deep learning.\end{tabular}                                                                                                                                                                                                                          & \begin{tabular}[c]{@{}l@{}}Task 1     Information not available.\\      Task 2     embeddings: BioBERT.\end{tabular}                                                                                  & \begin{tabular}[c]{@{}l@{}}Task 1     The title and  abstract of the paper   in the accepted format.\\      Task  2     The title and  abstract of the paper   in the accepted format.\end{tabular}   & \begin{tabular}[c]{@{}l@{}}Task 1     NamePre classification of papers based on inclusion probability (not   Available)\\      Range: Information not available.\\      Threshold: Information not available.\\      Task 2     Name:Pre classification of papers based on inclusion probability (not   Available)\\      Range: (0-1){[}Possible RCT, Not RCT{]}.\\      Threshold:  Information not   available.\end{tabular}                                                                                      & \begin{tabular}[c]{@{}l@{}}Task 1     Relevant papers: Information not available.\\      Irrelevant papers:Information not available.\\      Task 2     Not Applicable.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Task 1     Synchronous: the model runs in the background.     Task 2\\      Synchronous: the model runs in the   background.\end{tabular} & PICO identification: Highlights the   parts of a PICO  question in the   abstract.                                                                                                                                                                                                                                                                                                                                                                                                            & None                                                      \\
pitts.ai                  & Biomedicine    & Identification   of biomedical studies(RCTs) based on a pre-built classification model.                                                                                                                                                                                                                               & No   user interaction.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            & ML classifier   (Superivised Learning) based on SVM.                                                                                                                                                                                                                                                                                                                                                                                                & embeddings:SciBERT                                                                                                                                                                                    & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre classification of papers based on inclusion   probability (prediction probability).     Range: 0-1.\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                                                                                                                                                    & \begin{tabular}[c]{@{}l@{}}Relevant   papers:  Not Applicable.\\      Irrelevant papers:  Not Applicable.\end{tabular}                                                               & Synchronous: the   model runs in the background.                                                                                                                     & None                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & None                                                      \\
Rayyan                    & Any            & Classification   of relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML   classifier (Active Learning) based on SVM.                                                                                                                                                                                                                                                                                                                                                                                                     & bag   of words:ngrams                                                                                                                                                                                 & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability(score   probability)\\      Range: A 5 star scheme, the closer to 5 the    paper be consider as relevant\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                                                                                     & \begin{tabular}[c]{@{}l@{}}Relevant   papers: 5.\\      Irrelevant papers:5.\end{tabular}                                                                                            & Synchronous:   the model runs in the background.                                                                                                                     & \begin{tabular}[c]{@{}l@{}}Keywords   search: It searches by    keywords that could be highlighted;\\      Other searches: It   searches by author or publication year;\\      Boolean Operator: It searches by the combination of boolean operators(AND, OR,   NOT) with keywords.\end{tabular}                                                                                                                                                                                              & None                                                      \\
Research   Screener       & Any            & Classification   of relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML   classifier (Active Learning) based on unkown algorithm.                                                                                                                                                                                                                                                                                                                                                                                        & embeddings:   paragraph embedding                                                                                                                                                                     & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability(inclusion   probability)\\      Range: Information not available.\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                                                                                                                            & \begin{tabular}[c]{@{}l@{}}Relevant   papers: 1.\\      Irrelevant papers: Information not available.\end{tabular}                                                                   & Synchronous:   the model runs in the background.                                                                                                                     & None                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & None                                                      \\
RobotAnalyst              & Any            & Classification   of relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML   classifier (Active Learning) based on SVM.                                                                                                                                                                                                                                                                                                                                                                                                     & bag   of words: Information not available.                                                                                                                                                            & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability(inclusion   confidence)\\      Range: 0-1\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                                                                                                                                                    & Relevant   papers: Information not available.     Irrelevant papers: Information not available.                                                                                      & Synchronous:   the model runs in the background.                                                                                                                     & Topic   modelling: It assigned    a topic to a paper based on the    most recurrent terms which    could be shared by other papers; clustering: groups paper on the most common terms that are not overlap; Keywords search: searches by   keywords; term search: searches   by terms(noun phrases)  extracted from   the title and abstract; Other criterias: Document id, Publication Year, Author, Type of Publication,   Journal, Notes, Time of screening decision,    retrieval method; & None                                                      \\
RobotReviewer/RobotSearch & Biomedicine    & Identification of biomedical studies(RCTs)   based on a pre-built classification model.                                                                                                                                                                                                                               & No user interaction.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              & ML classifier (Active   Learning) based on SVM.                                                                                                                                                                                                                                                                                                                                                                                                     & embeddings:SciBERT                                                                                                                                                                                    & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability(prediction   probability).\\      Range: 0-1.\\      Threshold: Not Available.\end{tabular}                                                                                                                                                                                                                                                                                                                            & \begin{tabular}[c]{@{}l@{}}Relevant   papers: Not Applicable.\\      Irrelevant papers:Not Applicable.\end{tabular}                                                                  & Information not   available.                                                                                                                                         & PICO model:  It colour the  different PICO elements.                                                                                                                                                                                                                                                                                                                                                                                                                                          & Pending                                                   \\
SWIFT-Active   Screener   & Any            & Classification   of relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML   classifier (Active Learning) based on log-linear.                                                                                                                                                                                                                                                                                                                                                                                              & bag   of words: Information not available.                                                                                                                                                            & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability(inclusion   rate).\\      Range: 0-1.\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                                                                                                                                                        & \begin{tabular}[c]{@{}l@{}}Relevant   papers: 1.\\      Irrelevant papers:1.\end{tabular}                                                                                            & Asynchronous:   The model updates every  30 papers.   There must be a gap of 2 minutes between the last model built and the current   model built.                   & Keywords search: Basic search trough   keywords                                                                                                                                                                                                                                                                                                                                                                                                                                               & None                                                      \\
SWIFT-Review              & Biomedicine    & Classification   of relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML   classifier (Active Learning) based on log-linear.                                                                                                                                                                                                                                                                                                                                                                                              & bag   of words: Information not available.                                                                                                                                                            & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability(priority  ranking).\\      Range: 0-1.\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                                                                                                                                                       & \begin{tabular}[c]{@{}l@{}}Relevant   papers: 1.\\      Irrelevant papers:1.\end{tabular}                                                                                            & Synchronous:   the model runs in the background.                                                                                                                     & \begin{tabular}[c]{@{}l@{}}Keywords   search: Basic search trough keywords.     \\      Topic modelling: It assigned  a topic to a paper based on the  most recurrent terms which  could be shared by other papers; Keywor   search: searches by keywords or tags;\end{tabular}                                                                                                                                                                                                               & None                                                      \\
SysRev.com                & Any            & Classification   of relevant papers given a set of seed papers.                                                                                                                                                                                                                                                       & The   user has to rank papers as relevant and irrelevant.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & ML   classifier (Active Learning) based on a customized architecture similar to   cross attention.                                                                                                                                                                                                                                                                                                                                                  & Information not   available.                                                                                                                                                                          & The   title and  abstract of the paper in the   accepted format.                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}Name:Pre   classification of papers based on inclusion probability(prediction   probability).\\      Range: Information not available.\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                                                                                                                          & \begin{tabular}[c]{@{}l@{}}Relevant   papers: 30.\\      Irrelevant papers: 30.\end{tabular}                                                                                         & Asynchronous: The   model updates nightly.                                                                                                                           & None                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & None                                                     
\end{tabular}
\end{table}


==> tables/TableA2.tex <==
\begin{table}[]
  \caption{Tools for the extraction phase described according to the AI features}
    \label{tab:tools_described_ai_features_extraction}


\begin{tabular}{l|l|l|l|l|l|l|l}
Tool                      & Research Field                 & SLR Task                                                                                                                                              & Human   Interaction                                                                                                                                                                                            & Approach                                                                                                                                                                                                                                                                                          & Text   Representation                                                                                                           & Input               & Output                                                                                                                                                                                                                                                                                                                                                                       \\
RobotReviewer/RobotSearch & Biomedical                     & Identification of   risk of bias.                                                                                                                     & The user has to   upload the papers in PDF format                                                                                                                                                              & \begin{tabular}[c]{@{}l@{}}ML   classifier based on the combination of a    lineal model and Convolutional Neural Network (CNN) model. \\      The models are trained on a dataset made of sentences stating the level of   risk of bias  manually annotated for   each RCT.\end{tabular}         & \begin{tabular}[c]{@{}l@{}}Lineal Model     Bag of word: ngrams.     CNN Model\\      embeddings: embedding layer.\end{tabular} & Full-text paper.    & \begin{tabular}[c]{@{}l@{}}Name:   Risk of bias classification\\      Range: Low, High, Unclear(there is inssuficient information).\\      Threshold: Information not available.\end{tabular}                                                                                                                                                                                \\
ExaCT                     & Biomedical                     & NER of RCT.                                                                                                                                           & The user has to   upload the papers in HTML format                                                                                                                                                             & \begin{tabular}[c]{@{}l@{}}1.   ML classifier  based on SVM.\\      2. Rule base detection.\\      \\      The model predicts sentences similar    of the pretrained model. Then it selects the enties applying rule   based  of the 21 categories.\end{tabular}                                  & Bag   of words: ngrams.                                                                                                         & Full-text paper.    & \begin{tabular}[c]{@{}l@{}}Name:   Possible RCT entities.\\      Range: Not Applicable.\\      Threshold: Not Applicable.\end{tabular}                                                                                                                                                                                                                                       \\
Dextr                     & Environmental   Health Science & \begin{tabular}[c]{@{}l@{}}Task 1     NER of animal studies.\\      Task 2     Entity linking of animal studies.\end{tabular}                         & The has to upload the   papers in PDF, ris or Endnote format                                                                                                                                                   & \begin{tabular}[c]{@{}l@{}}Task 1     ML Classifier implementing a neural network model based on a bidirectional   LSTM with a Conditional Random Field (BI-LSTM-CRF) architecture.\\      Task 2     Customised Ontology.\end{tabular}                                                           & \begin{tabular}[c]{@{}l@{}}Task 1     embeddings: GloVe,ELMo.\\      Task 2     Not Applicable.\end{tabular}                    & Title and Abstracts & \begin{tabular}[c]{@{}l@{}}Task 1     Name: Possible animal entities.\\      Range: Information not    available.\\      Threshold: Information not    available.\\      \\      Task 2     Name: Relationships of animal models and exposures vs experimentas  ot    endpoints vs experiments.\\      Range: Not Applicable.\\      Threshold: Not Applicable.\end{tabular} \\
Iris.ai                   & Any                            & \begin{tabular}[c]{@{}l@{}}Task 1     NER of entities required by the user.\\      Task 2     Entity linking of the identified entities.\end{tabular} & The   user has to upload the PDF files or select them from his dataset. He has to   submit the Output Data Layout (ODL) which is a spreedsheet that  contains all the entities he wants the user   to extract. & \begin{tabular}[c]{@{}l@{}}Task 1     ML classifier  which algorithim is   unknow.\\      \\      Task 2     Uses a knowledge graph to represent the relations of within the entities on   the paper or between the entities of the table. The technical implementation   in unkown.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Task 1     embeddings: word embedding.\\      Task 2\\      Not Applicable.\end{tabular}             & Full-text paper.    & \begin{tabular}[c]{@{}l@{}}Task 1     Name: Possible entities based on a confidence interval.\\      Range: Not  Available.\\      Threshold: Not  Available.\\      \\      Task 2     Name: Relationships of entities\\      Range: Not Applicable.\\      Threshold: Not Applicable.\end{tabular}                                                                        
\end{tabular}
\end{table}

==> tables/generic_features.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[]

% \begin{tabular}{c|l|L{6cm}}
% \hline
% \textbf{C }                 & \textbf{Feature}                  & \textbf{Description} \\ \hline
% E                  & Free to use                       &   Whether the SLR tool is free to use or requires a premium subscription.                   \\ \hline
% \multirow{7}{*}{F} & Multiplatform                     &                      \\
%                    & Multiple user   roles             &                      \\
%                    & Multiple user   support           &                      \\
%                    & Project   auditing                &                      \\
%                    & Project   progress                &                      \\
%                    & Security                          &                      \\
%                    & Status of   software              &                      \\ \hline
% \multirow{6}{*}{R} & Automated full-text retrieval     &                      \\
%                    & Automated   search                &                      \\
%                    & Citations                         &                      \\
%                    & Manual   reference importing      &                      \\
%                    & Manually   attaching full-text    &                      \\
%                    & Reference   importing             &                      \\ \hline
% \multirow{5}{*}{S} & Deduplication                     &                      \\
%                    & Discrepancy   resolving           &                      \\
%                    & In-/excluding   references        &                      \\
%                    & Reference   labelling \& comments &                      \\
%                    & Screening   phases                &                      \\ \hline
% \multirow{3}{*}{D} & Exporting results                 &                      \\
%                    & Flow diagram   creation           &                      \\
%                    & Protocol                          &                      \\ \hline
% L                  & Living/updatable                  &                      \\ \hline
% \end{tabular}
% \end{table}


\begin{table}[]
\caption{List of generic features grouped based on their category.\label{tab:generic_features}}
\begin{tabular}{l|l|l}
\toprule
\textbf{Functionality}  & \textbf{Retrieval}                  & \textbf{Screening}                  \\
\midrule
Multiplatform           & Automated full-text retrieval       & Deduplication                       \\
Multiple user   roles   & Automated   search                  & Discrepancy   resolving             \\
Multiple user   support & Citations                           & In-/excluding   references          \\
Project   auditing      & Manual   reference importing        & Reference   labelling \&   comments \\
Project   progress      & Manually   attaching full-text      & Screening   phases                  \\
Security                & Reference   importing               &                                     \\
Status of   software    &                                     &                                     \\ \midrule
\textbf{Documentation}  & \textbf{Living System. Review} & \textbf{Economic}                   \\ \midrule
Exporting results       & Living/updatable                    & Free to use                         \\
Flow diagram   creation &                                     &                                     \\
Protocol                &                                     &   \\
\bottomrule
\end{tabular}
\end{table}

==> tables/temporary_table_mapping_features.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{THIS TABLE IS TEMPORARY HERE}
\begin{tabular}{r|l|l|l|c|c}
\toprule
\textbf{ID} & \textbf{Feature}             & \textbf{Provenance}        & \textbf{Type} & \textbf{Scree.} & \textbf{Extrac.} \\
\midrule
1           & Type of AI                   & \multirow{7}{*}{Previous}  & Overall       & y                           & y                            \\
2           & Algorithm                    &                            & Overall       & y                           & y                            \\
3           & Text Pre-processing          &                            & Technical     & y                           & n                            \\
4           & Human Interaction            &                            & Overall       & y                           & y                            \\
5           & Performance Metrics          &                            & NA            & n                           & n                            \\
6           & Input                        &                            & Technical     & y                           & y                            \\
7           & Output                       &                            & Technical     & y                           & y                            \\ \midrule
8           & research field               & \multirow{5}{*}{Francisco} & Overall       & y                           & y                            \\
9           & minimum requirement          &                            & Overall       & y                           & n                            \\
10          & model execution              &                            & Technical     & y                           & n                            \\
11          & pre-screening visualisation  &                            & visual        & y                           & n                            \\
12          & post-screening visualisation &                            & visual        & y                           & y       \\
\bottomrule
\end{tabular}
\end{table}
